NetReAct: Interactive Learning for Network Summarization

Generating useful network summaries is a challenging and important problem with several applications like sensemaking, visualization, and compression. However, most of the current work in this space do not take human feedback into account while generating summaries. Consider an intelligence analysis scenario, where the analyst is exploring a similarity network between documents. The analyst can express her agreement/disagreement with the visualization of the network summary via iterative feedback, e.g. closing or moving documents ("nodes") together. How can we use this feedback to improve the network summary quality? In this paper, we present NetReAct, a novel interactive network summarization algorithm which supports the visualization of networks induced by text corpora to perform sensemaking. NetReAct incorporates human feedback with reinforcement learning to summarize and visualize document networks. Using scenarios from two datasets, we show how NetReAct is successful in generating high-quality summaries and visualizations that reveal hidden patterns better than other non-trivial baselines.

==> 020preliminaries.tex <==



==> 030problem_formulation.tex <==
Our goal is to learn to generate network summaries which helps us in interactive visualization of networks.

\subsection{Interactive visualization task}
Collaborative visualization is an important area and has seen  growing research work in recent years \cite{bradel2014multi,bradel2011space}.  It helps in understanding large networks and making sense of them with the guidance of human feedback. One of the state-of-the-art methods in collaborative visulization is \starspire \cite{bradel2014multi}. It is a visual text analytics tool which leverages user semantic interactions on documents to give a high-quality relevancy-based document visualization. \starspire helps users to explore a document corpus effectively and find the information they need by reading the relevant documents as fast as possible. \starspire can be considered as a content-based recommendation system. For example, if the user opens a document and express her interest to it through the semantic interactions such as bookmarking or highlighting parts of it, \starspire visualizes similar documents on screen and recommend them to read. So, user can find the more relevant documents easier. Hence, one of the main tasks that \starspire accomplishes is to visualize relevant documents close to each other to recommend them and guide the user. Figure \ref{fig:starspire_pipeline} shows an overview of \starspire pipeline. 
\subsection{Overview of \starspire}
We can consider the \starspire task as a network $G(V, E, W)$ visualization for the purpose of recommendation. In $G(V, E, W)$,  $V$ is the set of documents, and $E$ is the set of edges representing the similarity relation between them, and $W$ is the set of edge weights representing the amount of similarity based on their word usage. \starspire uses a weighted, force-directed layout to place similar documents based on user interest nearer to each other in the 2-D visualization of $G$. The framework learns the user interest from its semantic interactions such as opening, minimizing, removing, annotating and highlighting documents. Note, the user interest can be captured by these semantic interactions. If $\Upsilon(i, j)$ is a function that shows the relevance of document $i$ to $j$ based on the user interest, the goal is to visualize the relevant documents with higher $\Upsilon(i, j)$ nearer to each other. More formally we can consider the \starspire task as follow,
\begin{problem}{\starspire Document Visualization}
\label{def:starspire}
\par\noindent
\textbf{Given} a document network  $G(V, E, W)$, and a relevance function $\Upsilon(\cdot, \cdot)$,
\par\noindent
\textbf{Generate} a graph visualization $\viz^* \in \mathbb{R}^{|V|\times 2}$ of $G$ in a 2-d space such that, 

\begin{align}
&\viz^* = \arg\min_{\viz} \sum_{i,j \in V} \Upsilon(i, j)\cdot \left[ F_{repulsive}(i,j) + F_{attractive}(i,j)\right] \\
&s.t. \qquad \forall_{i,j \in V} ||\viz(i) - \viz(j)||_2 >0\\ \notag
&\textsf{Where, }\\ \notag
&F_{repulsive}(i,j) = \frac{-1}{||\viz(i)-\viz(j)||}\\ \notag
&F_{attractive}(i,j)= ||\viz(i) - \viz(j)||^2
\end{align}
where, the constraint guarantees that there is not overlapping in the visualization \viz.
\end{problem}

This problem is challenging because it is hard to define the relevance function $\Upsilon$ which characterizes the user's interests. Also, each user has a unique interest which can also depend on the task.

\par\noindent
\textbf{Formal formulation}

\par\noindent
\textbf{Difference between our problem and \netgist}



==> notes.tex <==
Top to dos:

1) Writing
\begin{itemize}
    \item Justify the use of RL for the problem.
    \item Explain the difference/similarities between 'supernode' and 'document cluster'.
    \item Related work.
\end{itemize}

2) Experiments
\begin{itemize}
    \item Add baselines.
\end{itemize}
